DeepROCK: Error-controlled interaction detection in deep neural networks

The complexity of deep neural networks (DNNs) makes them powerful but also makes them challenging to interpret, hindering their applicability in error-intolerant domains. Existing methods attempt to reason about the internal mechanism of DNNs by identifying feature interactions that influence prediction outcomes. However, such methods typically lack a systematic strategy to prioritize interactions while controlling confidence levels, making them difficult to apply in practice for scientific discovery and hypothesis validation. In this paper, we introduce a method, called DeepROCK, to address this limitation by using knockoffs, which are dummy variables that are designed to mimic the dependence structure of a given set of features while being conditionally independent of the response. Together with a novel DNN architecture involving a pairwise-coupling layer, DeepROCK jointly controls the false discovery rate (FDR) and maximizes statistical power. In addition, we identify a challenge in correctly controlling FDR using off-the-shelf feature interaction importance measures. DeepROCK overcomes this challenge by proposing a calibration procedure applied to existing interaction importance measures to make the FDR under control at a target level. Finally, we validate the effectiveness of DeepROCK through extensive experiments on simulated and real datasets.

==> makefile <==
all: main.pdf

%.pdf: %.tex
	pdflatex $*.tex
	if ( grep -q bibliographystyle $*.tex ) ; then \
		bibtex $* ; \
		pdflatex $*.tex ; \
	fi
	pdflatex $*.tex

%.pdf: %.fig
	fig2dev -L pdftex -p dummyarg $*.fig $*.pdf

clean:
	rm -f *.dvi *.bbl *.aux *.blg *.log *.ps *.out


